Accelerator Control System at KEKB and the Linac

KEKB completed all of the technical milestones, and had offered important insights into the flavor structure of elementary particles, especially the CP violation. The accelerator control system at KEKB and injector linac was initiated by a combination of scripting languages at the operation layer and EPICS at the equipment layer. During the project many features were implemented to achieve extreme performance out of the machine. Especially the online linkage to the accelerator simulation played an essential role. In order to further improve the reliability and flexibility two major concepts were additionally introduced later in the project, namely the channel access everywhere and the dual-tier controls. Based on the improved control system a concept of virtual accelerators were realized that enables the single injector linac serve as three separate injectors to KEKB HER, LER and Photon Factory, respectively. Those control technologies are indispensable for the future particle accelerators.

==> Makefile <==
# Makefile for latex files
# K.Furukawa, Aug.29.1998.
# K.Furukawa, Jun.9.2000.  add ps2pdf/acroread
# K.Furukawa, Aug.8.2000.  for linac2000
# K.Furukawa, May.6.2001.  for appi2001
# K.Furukawa, Nov.5.2001.  for NIM
# K.Furukawa, Aug.20.2002. adding clean1,realclean1, directory for cygwin
# K.Furukawa, Oct.2.2003.  adding pdf2 and ps2pdf compression rules
# K.Furukawa, Jul.2.2006.  dvips -j0 -ta4
# K.Furukawa, Oct.18.2008. dvips -j0 -ta4 -K
# K.Furukawa, Nov.25.2012. dvipdfmx for hyperref, instead of dvips/ps2pdf
#
# @(#) Makefile.tex v2.6.0 k.furukawa, aug.1998-nov.2012.
#
##########
# Please add path to tex binaries before you run make
##########
#
# TEXBIN = /usr/new/pkg/teTeX-1.0.5/bin
# TEXBIN = /usr/new/pkg/teTeX-2.0.2/bin
# MISCBIN = /usr/new/bin

# for cygwin
# TEXBIN = /usr/bin
# MISCBIN = /usr/bin

# for darwin
# TEXBIN = /sw/bin
# MISCBIN = /sw/bin

# should add PATH to programs

# LATEX = platex
LATEX = ${TEXBIN}latex
DVIPS = ${TEXBIN}dvips
DVIPDFMX = ${TEXBIN}dvipdfmx
# PS2PDF = ps2jpdf
# PS2PDF = ${MISCBIN}/ps2pdf
# PS2PDF = ${MISCBIN}/ps2pdf13
# PS2PDF = ${MISCBIN}/ps2pdfwr -dCompatibilityLevel=1.3 -dCompressPages=false
PS2PDF = ${MISCBIN}ps2pdfwr -dCompatibilityLevel=1.3 \
 -dUseFlateCompression=true \
 -dAutoFilterGrayImages=false \
 -dAutoFilterColorImages=false \
 -dGrayImageFilter=/FlateEncode \
 -dColorImageFilter=/FlateEncode
PS2PDF2 = ${MISCBIN}ps2pdfwr -dCompatibilityLevel=1.3 
PDFLATEX = ${TEXBIN}pdflatex
ACROREAD = acroread
% FILE = l5

# delete the default suffixes
.SUFFIXES:

.SUFFIXES: .ps .aux .tex .dvi .pdf-ps .pdf

# phony targets
.PHONY:	all clean clean1 realclean realclean1

# preserve intermediate targets
.PRECIOUS:	%.ps %.dvi %.ind %.idx %.aux %.toc %.pdf

all:	${FILE}.pdf

%.ps:	%.dvi
	@echo '### dvips ###'
	${DVIPS} -j0 -ta4 -K -D600 -o $@ $<

%.dvi:	%.aux
	@echo '### latex 2nd ###'
	${LATEX} $*.tex

%.aux:	%.tex
	@echo '### latex 1st ###'
	${LATEX} $*.tex
	rm $*.dvi

# pdflatex does not support eps
# see texmf/tex/latex/graphics/pdftex.def
%.pl-pdf:	%.aux
	@echo '### pdflatex ###'
	ln -s $*.tex $*.pl.tex
	ln -s $*.aux $*.pl.aux
	${PDFLATEX} $*.pl.tex
	-mv $*.pl.pdf $*.pl-pdf
	-rm $*.pl.tex $*.pl.aux

# %.pdf:	%.ps
#	@echo '### ps2pdf ###'
#	${PS2PDF} $<

%.pdf:	%.dvi
	@echo '### dvipdfmx ###'
	${DVIPDFMX} $<

%.pdf2:	%.ps
	${PS2PDF2} $<

# someone said it's better, but i don't think so
# %.pdf:	%.dvi
# 	@echo '### dvi2pdf ###'
# 	${DVIPS} -P pdf -G0 $<
# 	${PS2PDF} $*.ps

%.pdf-ps:	%.pdf
	@echo '### acroread ###'
	${ACROREAD} -toPostScript -level2 -size a4 -pairs $< $*.pdf-ps

# this cancels the built-in rule from .tex to .dvi
%.dvi:	%.tex


# static rules
#
#${FILE}.ps:	${FILE}.dvi
#	${DVIPS} -D600 -o $@ ${FILE}.dvi
#
#${FILE}.aux:	${FILE}.tex
#	${LATEX} ${FILE}.tex
#	rm ${FILE}.dvi
#
#${FILE}.dvi:	${FILE}.tex ${FILE}.aux
#	${LATEX} ${FILE}.tex
#

realclean:	clean
	find . -regex '.*\.\(ps\|pdf\|pdf2\|pdf-ps\)' \
	-mtime -2 -exec rm {} \;

clean:	
	find . -regex \
	'.*\.\(dvi\|log\|aux\|toc\|idx\|ind\|ilg\|bbl\|blg\|out\)' \
	-mtime -2 -exec rm {} \;

realclean1:	clean1
	find . -regex '.*\.\(ps\|pdf\|pdf2\|pdf-ps\)' \
	-exec rm {} \;

clean1:	
	find . -regex \
	'.*\.\(dvi\|log\|aux\|toc\|idx\|ind\|ilg\|bbl\|blg\|out\)' \
	-exec rm {} \;

